Unifying Unsupervised Graph-Level Anomaly Detection and Out-of-Distribution Detection: A Benchmark

To build safe and reliable graph machine learning systems, unsupervised graph-level anomaly detection (GLAD) and unsupervised graph-level out-of-distribution (OOD) detection (GLOD) have received significant attention in recent years. Though those two lines of research indeed share the same objective, they have been studied independently in the community due to distinct evaluation setups, creating a gap that hinders the application and evaluation of methods from one to the other. To bridge the gap, in this work, we present a \underline{\textbf{U}}nified \underline{\textbf{B}}enchmark for unsupervised \underline{\textbf{G}}raph-level \underline{\textbf{O}}OD and anoma\underline{\textbf{L}}y \underline{\textbf{D}}etection (\ourmethod), a comprehensive evaluation framework that unifies GLAD and GLOD under the concept of generalized graph-level OOD detection. Our benchmark encompasses 35 datasets spanning four practical anomaly and OOD detection scenarios, facilitating the comparison of 18 representative GLAD/GLOD methods. We conduct multi-dimensional analyses to explore the effectiveness, OOD sensitivity spectrum, robustness, and efficiency of existing methods, shedding light on their strengths and limitations. Furthermore, we provide an open-source codebase (https://github.com/UB-GOLD/UB-GOLD) of \ourmethod to foster reproducible research and outline potential directions for future investigations based on our insights.

==> Sections/1_intro_v1.5.tex <==
\kz{My thoughts:
1. You can first talk about graph-level anomaly detection
2. Then say in the meantime, another line of research graph OOD detection has received increasing research attention, but indeed most of them are unsupervised,which shares the same goal with graph-level anomaly detection.
3. However, those two lines of research are studied independently with different evaluations. To bridge the gap, we follow the definition of generalized OOD detection and develop this benchmark.
4. Talk about how we evaluate. 
}

With the ubiquity of graph data, graph machine learning has been widely adopted in various scientific and industrial fields, ranging from bioinformatics to social networks. Most existing approaches operate under the closed-world assumption, where all test samples are assumed to come from the same distribution as the training data, known as ``in-distribution (ID)''; however, such an assumption rarely holds in real-world scenarios where out-of-distribution (OOD) samples from different distributions can often appear~\cite{yang2022openood}. Ideally, a reliable graph machine learning system should not only accurately predict known ID samples but also recognize ``unknown'' OOD samples during inference~\cite{liu2023goodd}. More recently, graph-level OOD detection (GLOD) aiming at identifying whether each graph sample in a test set is ID or OOD has drawn increasing attention due to its critical role in real-world high-stakes applications such as drug discovery and cyber-attack detection~\cite{shen2024pgrmood,ji2023drugood,ju2024survey}. While a few post-hoc GLOD methods~\cite{guo2023aagod,wang2024goodat} rely on a well-trained graph classifier, existing GLOD methods~\cite{liu2023goodd,shen2024pgrmood,ding2023sgood} predominately follow an unsupervised paradigm, where a specific OOD detection model is trained on ID data, and then predicts a score for each test sample to indicate its ID/OOD status. Since GLOD emerged in late 2022, the field has seen only a few methods~\cite{liu2023goodd,shen2024pgrmood,guo2023aagod,wang2024goodat,ding2023sgood,li2022graphde}, highlighting the expectation for more powerful, robust, and comprehensive solutions to address this cutting-edge research challenge\kz{is this related to benchmark? You may rewrite this}. 

% To address this, graph-level OOD detection (GLOD)\kz{why suddenly graph-level? Maybe give some applications can help} is an emerging research direction that aims to identify whether each graph sample in a test set is ID or OOD. 


In contrast to GLOD, graph-level anomaly detection (GLAD) is a more well-explored research problem, with numerous solutions ranging from shallow detectors~\cite{breunig2000lof,amer2013enhancing_ocsvm} to deep graph neural network (GNN)-based approaches~\cite{ma2022deep_glocalkd,ijcai2022p305_ocgtl}. Due to the inherent connections between GLOD and GLAD problems, it is natural to adopt GLAD methods to solve GLOD tasks~\cite{liu2023goodd,li2022graphde}. Firstly, GLAD shares a similar goal with GLOD: identifying graph samples that significantly differ from normal patterns. In fact, the abnormality of samples can also be regarded as a kind of semantic distribution shift. Recent survey and benchmark papers~\cite{yang2022openood,yang2021survey} identify anomaly detection and OOD detection as two branches under the concept of ``generalized OOD detection'', which further highlights the close conceptual connection between GLOD and GLAD tasks. Moreover, most GLAD studies follow an unsupervised paradigm, without the requirement of anomaly samples for model training~\cite{ma2022deep_glocalkd,ijcai2022p305_ocgtl,liu2023signet}. This makes it feasible to apply these unsupervised GLAD methods directly to unsupervised GLOD in practice. \kz{this paragraph is kind of too wordy} 
Considering their similarities, a natural question arises: 

\vspace{-2mm}
\begin{center}
    \textbf{\textit{Can we frame GLOD and GLAD as a unified research problem, \\ enabling state-of-the-art (SOTA) methods for one problem to be applied in the other?}}
\end{center}
\vspace{-2mm}

% \begin{center}
%     \textbf{\textit{Can the state-of-the-art GLAD methods effectively handle the GLOD problem, and vice versa?}}
% \end{center}

\begin{figure*}[!t]
% \vspace{-6mm}
  \includegraphics[width=1\textwidth]{Figs/intro.pdf}
  \vspace{-6mm}
  \caption{Diagram of generalized OOD detection scenarios supported by \ourmethod.}
  \vspace{-4mm}
  \label{fig:sketch}
\end{figure*}

While few studies~\cite{liu2023goodd,guo2023aagod} have demonstrated through experiments that methods from one field can serve as baselines in the other, most existing research typically addresses GLOD and GLAD issues independently. To fill the gap, we develop a \textbf{\underline{U}}nified \textbf{\underline{B}}enchmark for unsupervised \textbf{\underline{G}}raph-level \textbf{\underline{O}}OD and anoma\textbf{\underline{L}}y \textbf{\underline{D}}etection (\ourmethod for short). %, including 27(?) datasets from 4 GLOD/GLAD scenarios for comprehensive evaluation. 
As shown in Fig.~\ref{fig:sketch}, we unify GLOD and GLAD as ``generalized graph-level OOD detection problem'', and consider 2 GLOD scenarios and 2 GLAD scenarios for comprehensive evaluation. 
% As shown in Fig.~\ref{fig:sketch}, under the umbrella of generalized graph-level OOD detection, \ourmethod covers 2 GLOD scenarios and 2 GLAD scenarios. 
For GLOD problem that emphasizes the distribution shift between ID and OOD samples, we consider two scenarios with different distribution shifts, i.e., \textbf{inter-dataset shift} and \textbf{intra-dataset shift}. Specifically, the former simulates distribution shifts by drawing ID and OOD samples from different datasets within the same domain~\cite{liu2023goodd,sehwag2021ssd}, while the latter refers to datasets with intrinsic distribution shifts regarding graph sizes or molecular scaffolds~\cite{gui2022good}. For GLAD problem that aims to detect graph samples with semantic abnormality, we explore scenarios with \textbf{organic anomaly} %\kz{real-world or organic anomaly?}
and \textbf{class-based anomaly}%\kz{minority class anomaly?}
.  Specifically, the first type of dataset inherently includes semantic anomalies, while the second type treats samples from one class (usually the minority class) as anomalies. Based on 35 datasets from the above 4 scenarios, we establish a comprehensive benchmark to fairly compare 18 GLOD and GLAD methods under a unified experimental setting, exploring the effectiveness of SOTA approaches across diverse scenarios and domains.

Apart from comparing performance, we further investigate the characteristics of GLOD/GLAD methods in terms of three dimensions: generalizability, robustness, and efficiency, through extensive experiments. For \textbf{generalizability}, we test a well-trained GLOD/GLAD model on OOD data with varying degrees of distribution shift, investigating each method's ability to identify both near-OOD and far-OOD samples. For \textbf{robustness}, we introduce varying proportions of OOD samples into the training data to observe the impact of noisy ID data on the performance of existing methods. For \textbf{efficiency}, \ourmethod performs a detailed evaluation of representative GLOD/GLAD approaches, focusing on time and space complexity. %For \textbf{parameter sensitivity}, we compare the performance of each method under default and optimal hyper-parameter settings, showcasing the stability and adaptability of each approach to different parameter configurations. 
At the end of this paper, we also discuss the future directions of this emerging research direction. To sum up, the main contribution of this paper is three-fold: 

\begin{itemize}[leftmargin=*,noitemsep]
    \item \textbf{Comprehensive benchmark.} We introduce \ourmethod, the first comprehensive and unified benchmark for GLOD and GLAD. \ourmethod compares 18 representative GLOD/GLAD methods across 35 datasets from four practical OOD and anomaly detection scenarios.
    \item \textbf{Multi-dimensional analysis.} To explore their ability and limitations, we conduct a systematic analysis of existing methods from four dimensions, encompassing the generalizability to near-OOD and far-OOD, the robustness against unreliable training data, the efficiency in terms of time and memory usage, and the sensitivity to hyper-parameter tuning. 
    \item \textbf{Unified Codebase and future directions.} To facilitate future research and quick implementation, we provide an open-source codebase for \ourmethod. We also outline potential directions based on our findings to inspire future research.
\end{itemize}

\noindent\textbf{Key findings.} Through comprehensive comparison and analyses, we have the following observations: 1) GLAD-based and GLOD-based Models are Effective Across Both Tasks; 2) Excellence in AUROC Does Not Mask AUPRC and FPR95 Deficiencies; 3) Larger Differences from ID Samples Facilitate Detection; 4) Performance Degradation with Increasing OOD Contamination; 5) Great E2E methods outperform 2-Step methods from performance to time and space consumption. 



==> Sections/1_intro_v1.tex <==
Graphs are a ubiquitous structure in a multitude of scientific and industrial fields, ranging from bioinformatics to social networks.
Effective machine learning on graphs necessitates robust graph-level anomaly detection (GL-A-D) and out-of-distribution detection (GL-OOD-D) capabilities to ensure accurate and reliable applications. 
GLAD aims to pinpoint graph instances that deviate significantly from typical patterns, critical for tasks such as identifying pathological structures in neurological data or anomalies in structural engineering data. 
Conversely, OODD focuses on identifying graph samples that diverge from the training distribution, crucial for real-world deployments where training conditions cannot encompass future variations.

Both GLAD and OODD share a common goal: identifying graph data that differ from a 'norm'. 
In fact, existing research has demonstrated through experiments that methods from one field can serve as strong baselines in the other. However, they are often tackled separately. This separation overlooks their conceptual and methodological overlaps, such as their reliance on similar statistical metrics for performance evaluation and their common need for handling diverse and complex data structures. For instance, in drug discovery, it is paramount for models not only to recognize known toxicological profiles (GLAD) but also to be adept at identifying novel compounds that may not conform to the training set (GLOODD). Despite these similarities, there is a stark absence of a unified benchmark that integrates both GLAD and GLOODD paradigms, which limits the cross-pollination of ideas and techniques between these fields.

The development of a unified benchmark that integrates both GLAD and GLOODD paradigms is essential. Such a benchmark would facilitate the evaluation and comparison of methods across both domains, promoting the transfer of innovative approaches and fostering a deeper understanding of their interdependencies. By addressing this gap, researchers can more effectively develop and refine models that excel in detecting both in-distribution anomalies and out-of-distribution instances.

Current benchmarks in graph-level anomaly detection and out-of-distribution detection confront significant challenges that obstruct the creation of universally effective models.  A primary concern is the varied applications and validations across different datasets, leading to an inconsistent understanding of model performance. In GLAD, benchmarks often employ "Class-based" or "Real anomaly-based" datasets, in which anomalies are intrinsically integrated into the data.  In contrast, GLOODD typically deals with "Dataset-based" and "Shift-based" scenarios, where anomalies are defined by differences across distributions or result from shifts within the dataset itself. This disparity in how datasets are utilized complicates the development of uniform partitioning methods, thus hindering the ability to accurately assess and compare the effectiveness of models across these domains.

To effectively address the discrepancies in current graph-level anomaly detection (GLAD) and out-of-distribution detection (GLOODD) benchmarks, we propose a new, comprehensive benchmark titled "Unifying Graph-Level Anomaly and OOD Detection." This benchmark aims to standardize evaluation by employing consistent dataset partitions and a unified set of metrics—AUROC, AUPRC, and FPR95—across a variety of graph-based data scenarios, including class-based, real anomaly-based, dataset-based, and shift-based anomalies. By offering a standardized framework for fair and transparent comparisons, this initiative seeks to enhance the robustness and applicability of detection methods, fostering the development of models that are effective across diverse graph contexts and advancing the field towards more generalized solutions.


\begin{itemize}
    \item \textbf{Unified Benchmark Development:} The introduction of "Unifying Graph-Level Anomaly and OOD Detection" serves as a pioneering effort to merge GLAD and GLOODD into a single evaluation framework. This approach standardizes the assessment process across these domains, ensuring that models can be robustly tested against a variety of graph scenarios, including class-based, real anomaly-based, dataset-based, and shift-based scenarios.
    
    \item \textbf{Standardization and Fair Comparison:} By employing unified metrics such as AUROC, AUPRC, and FPR95, this benchmark standardizes the evaluation of anomaly and out-of-distribution detection models. This not only facilitates fair and transparent comparisons but also helps in systematically understanding model strengths and weaknesses across different types of graph data.
    
    \item \textbf{Consistent Dataset Partitions:} A major advancement is the establishment of consistent dataset partitions which address previous discrepancies in how datasets were utilized and validated. This uniform partitioning allows for more accurate and comparable assessments of model efficacy, enhancing the reliability of benchmarks across diverse graph contexts and applications.
    
\end{itemize}

==> Sections/1_intro_v3.tex <==
With the ubiquity of graph data, graph machine learning has been widely adopted in various scientific and industrial fields, ranging from bioinformatics to social networks~\cite{xia2021graph,wu2020comprehensive}. 
As one of the representative graph learning tasks, graph-level anomaly detection (GLAD) has been widely studied to identify abnormal graphs that show significant dissimilarity from the majority of graphs in a collection~\cite{ma2022deep_glocalkd,zhang2022dual_igad}. GLAD task is crucial in various real-world applications, such as toxic molecule recognition and pathogenic brain mechanism discovery~\cite{jiang2021ggl,mirakhorli2020new}. Due to the high cost of data labeling, existing GLAD studies generally follow an unsupervised paradigm, eliminating the requirement of labeled anomaly samples for model training~\cite{ma2022deep_glocalkd,ijcai2022p305_ocgtl,liu2023signet}.

In the meantime, another line of research -- graph-level out-of-distribution detection (GLOD) -- has drawn increasing attention in the research community lately. GLOD aims to identify whether each graph sample in a test set is in-distribution (ID), meaning it comes from the same distribution as the training data, or out-of-distribution (OOD), indicating it comes from different distributions. Considering the universality of distribution shift in open-world data, GLOD plays an important role in real-world high-stakes applications such as drug discovery and cyber-attack detection~\cite{shen2024pgrmood,ji2023drugood,ju2024survey}. Though a few post-hoc GLOD methods~\cite{guo2023aagod,wang2024goodat} that rely on a well-trained graph classifier have been proposed, most of the existing GLOD methods~\cite{liu2023goodd,shen2024pgrmood,li2022graphde}  follow an unsupervised paradigm, where a specific OOD detection model is trained on unlabeled ID data, and then predicts a score for each test sample to indicate its ID/OOD status. In essence, unsupervised GLOD and unsupervised GLAD share the same goal, suggesting that research in one area could potentially be applied to solve problems in the other.  Recent survey and benchmark papers~\cite{yang2022openood,yang2021survey} also identify anomaly detection and OOD detection as two branches under the concept of ``generalized OOD detection'', which further highlights the close conceptual connection between GLOD and GLAD tasks.  

Despite the inherent connection between the problems of unsupervised GLAD and GLOD, those two research sub-areas have been studied independently in the literature and have distinct evaluation setups. To fill the gap, in this paper, we develop a \textbf{\underline{U}}nified \textbf{\underline{B}}enchmark for unsupervised \textbf{\underline{G}}raph-level \textbf{\underline{O}}OD and anoma\textbf{\underline{L}}y \textbf{\underline{D}}etection (\ourmethod for short). 
As shown in Fig.~\ref{fig:sketch}, we unify GLAD and GLOD as ``generalized graph-level OOD detection problem'', and consider 2 GLOD scenarios and 2 GLAD scenarios for comprehensive evaluation. 
For GLAD task that aims to detect graph samples with semantic abnormality, we explore scenarios with \textbf{organic anomaly} and \textbf{class-based anomaly}.  Specifically, the first type of dataset inherently includes semantic anomalies, while the second type treats samples from one class (usually the minority class) as anomalies. 
For GLOD task that emphasizes the distribution shift between ID and OOD samples, we consider two scenarios with different distribution shifts, i.e., \textbf{inter-dataset shift} and \textbf{intra-dataset shift}. Specifically, the former simulates distribution shifts by drawing ID and OOD samples from different datasets within the same domain~\cite{liu2023goodd,sehwag2021ssd}, while the latter refers to datasets with intrinsic distribution shifts regarding graph sizes or molecular scaffolds~\cite{gui2022good}. Based on 35 datasets belonging to 4 types, we establish a comprehensive benchmark to fairly compare 16 GLAD and GLOD methods under a unified experimental setting, exploring the {effectiveness} of state-of-the-art (SOTA) approaches across diverse scenarios and domains.

Apart from comparing performance, we further investigate the characteristics of GLAD/GLOD methods in terms of three dimensions: generalizability, robustness, and efficiency, through extensive experiments. For \textbf{generalizability}, we test a well-trained GLAD/GLOD model on OOD data with varying degrees of distribution shift, investigating each method's ability to identify both near-OOD and far-OOD samples. For \textbf{robustness}, we introduce varying proportions of OOD samples into the training data to observe the impact of noisy ID data on the performance of existing methods. For \textbf{efficiency}, we perform efficiency evaluations for representative GLAD/GLOD approaches, focusing on time and space complexity. 
At the end of this paper, we discuss the future directions of this emerging research direction. To sum up, the main contribution of this paper is three-fold: 

\begin{itemize}[leftmargin=*,noitemsep]
    \item \textbf{Comprehensive benchmark.} We introduce \ourmethod, the first comprehensive and unified benchmark for GLAD and GLOD. \ourmethod compares 16 representative GLAD/GLOD methods across 35 datasets from four practical anomaly and OOD detection scenarios.
    \item \textbf{Multi-dimensional analysis.} To explore their ability and limitations, we conduct a systematic analysis of existing methods from multiple dimensions, encompassing the generalizability to near-OOD and far-OOD, the robustness against unreliable training data, and the efficiency in terms of time and memory usage. 
    \item \textbf{Unified Codebase and future directions.} To facilitate future research and quick implementation, we provide an open-source codebase for \ourmethod. We also outline potential directions based on our findings to inspire future research.
\end{itemize}

\noindent\textbf{Key findings.} Through comprehensive comparison and analyses, we have the following remarkable observations: 
1) The SOTA GLAD/GLOD methods show excellent performance across tasks; 
2) Near-OOD samples are harder to detect compared to far-OOD samples; 
3) Most methods are vulnerable to the perturbations of training sets; and 
4) Certain end-to-end methods outperform 2-step methods in terms of both performance and computational costs. 


==> Sections/4_exp_v1.tex <==
In this section, we detail the experimental setup and discuss the results obtained from evaluating the performance of 16 GLOD and GLAD methods using the \ourmethod benchmark. Our experiments are structured around four pivotal research questions, aiming to dissect the effectiveness, robustness, and efficiency of these methods under various conditions and scenarios.

\textbf{RQ1: How do different GLOD and GLAD methods perform under various anomaly scenarios and distribution shifts?}

\textbf{Experiment Design:}
We systematically assess the methods across four distinct scenarios: inter-dataset shifts, intra-dataset shifts, real anomalies, and class-based anomalies. Performance is quantified using AUROC, AUPR, and FPR95 metrics, offering a comprehensive evaluation of each method's capacity to handle diverse and challenging datasets effectively. For each method and dataset, we report the mean performance from 5 runs, both with optimally tuned hyperparameters via random search and with default hyperparameter settings\footnote{Default hyperparameter settings sourced from the original publications of each method.}. This dual-parameter testing approach ensures robust and reproducible results by reflecting both ideal and practical usage conditions.


\begin{table}[ht]
\centering
\caption{Dataset statistics including ID Train, ID Test, Near OOD, and Far OOD counts. Additionally, Unseen Class (UC), Unseen Dataset (UD), Near Size (NS), and Far Size (FS).}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
\textbf{Data} & \textbf{ID Train} & \textbf{ID/Near/Far Test} & \textbf{Near OOD} & \textbf{Far OOD} \\
\midrule
AIDS    & 1280 & 80 & AIDS(UC) & DHFR(UD)\\
BZR     & 69   & 17 & BZR(UC) & COX2(UD)\\
ENZYMES & 400  & 20 & ENZYMES(UC) & PROTEINS(UD)\\
\midrule
GOOD-ZINC-Size & 1000  & 500 & ZINC(NS) & ZINC(FS)\\
\bottomrule
\end{tabular}}
\label{tab:near_far}
\end{table}

\textbf{RQ2: How effectively do GLOD and GLAD methods distinguish between near-OOD and far-OOD conditions?}

\textbf{Experiment Design:}
% To ensure a fair and unbiased evaluation of the differential performance of GLOD and GLAD methods in handling near and far OOD conditions, we have configured two distinct scenarios:
To rigorously evaluate the performance of GLOD and GLAD methods in handling near and far OOD conditions, we have implemented a distinct partitioning strategy for this research question. Unlike the setup in RQ1, here we ensure that the number of samples in the Near OOD, Far OOD, and ID Test groups are precisely equal, detailed in Table~.\ref{tab:near_far}. This balanced configuration is designed to provide a fair comparison across different degrees of out-of-distribution scenarios, and it includes two specific setups:

\begin{itemize}[leftmargin=*]\setlength{\itemsep}{5pt}

\item Class-based Anomaly Scenario: We utilize the class-based anomaly partitioning method to set the ID Train and ID Test, along with the Near OOD Test. The Far OOD Test employs datasets from the Inter-Dataset Shift category, representing more significant deviations.

\item Size-based Scenario: We maintain the same ID Train and ID Test groupings of Intra-Dataset Shift. However, for the Near OOD and Far OOD tests, we categorize the samples based on differing graph sizes, with smaller sizes representing Near OOD and larger sizes for Far OOD.

\end{itemize}

These scenarios are designed to rigorously test the capability of GLOD and GLAD methods to recognize and differentiate between subtle and substantial distribution shifts, thereby assessing their effectiveness in realistic and challenging environments.

\begin{table}[ht]
\centering
\caption{Dataset statistics including ID Train, ID Train with different perturbation levels, ID Test, and OOD Test counts.}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\textbf{Data} & \textbf{ID Train} & \textbf{ID Train (10\%)} & \textbf{ID Train (20\%)} & \textbf{ID Train (30\%)} & \textbf{ID Test} & \textbf{OOD Test} \\
\midrule
BZR      & 69  & 76  & 82  & 89  & 17  & 44 \\
PROTEINS & 360 & 374 & 387 & 400 & 90  & 93 \\
COX2     & 81  & 89  & 96  & 103 & 21  & 51 \\
\bottomrule
\end{tabular}}

\label{tab:perturbation}
\end{table}

\textbf{RQ3: How does the inclusion of  OOD samples in the ID train affect the robustness and performance of GLOD and GLAD?}

\textbf{Experiment Design:}
In this study, we investigate the robustness of GLOD and GLAD methods against the contamination of the ID training set with OOD samples. We begin by partitioning the OOD test dataset, randomly selecting 30\% of its samples to be mixed into the ID training set. The remaining 70\% of the OOD test dataset is kept intact for performance evaluation. This procedure is repeated to create four distinct experimental groups where 0\%, 10\%, 20\%, and 30\% of the originally selected OOD samples are added to the ID training dataset. These modifications allow us to systematically explore how progressively increasing the proportion of OOD samples within the ID training set affects the methods' ability to identify and differentiate true OOD instances during testing accurately.

\textbf{RQ4: Are the GLOD and GLAD methods efficient in terms of computational resources and processing time?}

\textbf{Experiment Design:}
We evaluate the computational efficiency of GLOD and GLAD methods using default hyperparameter settings provided in their original publications. Our assessment focuses on two main aspects:
\begin{itemize}[leftmargin=*]\setlength{\itemsep}{5pt}

\item Time Efficiency: We record the average time each method takes to achieve the best results across all datasets, offering insight into their processing speed.

\item Resource Usage: We monitor the average CPU and GPU consumption for each method during experiments, which helps determine their demand for computational resources.


\end{itemize}

This setup allows us to measure the methods' efficiency directly and reliably, reflecting their practicality for real-world application.

\subsection{Performance Comparison (RQ1)}
We present the performance of all methods across 35 datasets in Table~\ref{tab:AUROC_optimization} and Fig.~\ref{fig:combined}. Below, we highlight the key findings derived from these tables.

$\rhd$ \textbf{GLAD-based and GLOD-based Models are Effective Across Both Tasks}. The results in Table~\ref{tab:AUROC_optimization} highlight the versatility and effectiveness of both GLAD-based and GLOD-based models when applied across these two distinct yet related tasks. 
Notably, the GLAD-based model SIGNET demonstrates impressive performance in GLOD tasks (highlighted in green and yellow sections), achieving SOTAs in several datasets. 
This performance underscores the potential of GLAD-based methods to effectively address the challenges posed by OOD detection at the graph level.
Conversely, the GLOD-based model GOOD-D, while not achieving SOTAs in GLAD tasks (highlighted in red and blue sections), still performs admirably, securing an overall Rank.2. This performance illustrates the robustness and adaptability of GLOD-based methods in handling anomaly detection scenarios. The ability of these models to excel beyond their primary design scope highlights the potential for a unified approach in GLAD and GLOD.

$\rhd$ \textbf{Excellence in AUROC Does Not Mask AUPRC and FPR95 Deficiencies}. 
From Fig.~\ref{fig:combined} and Table~\ref{AUPRC_FPR95_optimization}, we can observe distinct differences in the stability of performance metrics across the models. While AUROC scores generally exhibit stability, with models like CVTGOD, GOOD-D, and SIGNET consistently achieving high median values, the AUPRC and FPR95 metrics reveal more variability and the presence of outliers. This indicates that models performing well in overall discrimination (AUROC) may struggle with precision-recall trade-offs and maintaining low false positive rates at high true positive rates, which are crucial for GLOD and GLAD tasks. The variability and outliers in AUPRC scores suggest that many models face challenges maintaining high precision and recall, crucial for reliably detecting anomalies and out-of-distribution instances where positive cases are rare. Similarly, the significant variability and poor performance in FPR95 scores highlight the difficulty in balancing sensitivity and specificity. This is particularly important in practical applications where false alarms can have significant consequences.


These findings validate the concept of unifying GLAD and GLOD tasks within a single benchmark framework. This unified framework simplifies the evaluation process and promotes the creation of more versatile and robust models. Evaluating using AUROC, AUPRC, and FPR95 metrics underscores the strengths and limitations of various GLOD and GLAD methods. While AUROC provides a stable measure of overall discriminative ability, AUPRC and FPR95 offer critical insights into model performance specific to the unified tasks. These findings highlight the importance of a multi-metric evaluation approach, guiding the development of more robust and versatile anomaly detection systems.


\begin{figure*}[!t]
  \centering
  \includegraphics[width=0.9\textwidth]{Figs/AUROC_AUPRC_FPR95_combined.pdf}
  \vspace{-4mm}
  \caption{Performance Metrics across Different Models.}
  \vspace{-4mm}
  \label{fig:combined}
\end{figure*}


\begin{table}[htbp]
\centering
\caption{Comparison of the AUROC score of each model with optimal hyperparameters through random search. The best results are highlighted in bold. In the last column, Ave. signifies the average rank across all datasets. 
% while Imp. denotes the absolute increase in this average score when compared to the default hyperparameters. 
Results for other metrics can be found in Appendix and Table.}
\label{tab:AUROC_optimization}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}l|cccc|cccc|cccccc|cc@{}}
\toprule
\rowcolor{gray!30} 
AUROC & PK-SVM & PK-iF & WL-SVM & WL-iF & IG-SVM & IG-iF & GCL-SVM & GCL-iF & OCGIN & GLocalKD & OCGTL & SIGNET & GLADC & CVTGAD & GOOD-D & GraphDE \\ 
\midrule
\rowcolor{red!20}
p53 & 49.17 & 54.05 & 57.69 & 54.40 & 68.11 & 60.85 & 68.61 & 64.6 & 68.35 & 65.43 & 67.58 & 68.10 & 65.82 & 69.4 & 67.82 & 62.59 \\
\rowcolor{red!20}
HSE & 60.72 & 56.49 & 63.27 & 52.98 & 60.33 & 22.77 & 67.40 & 63.95 & 71.42 & 60.21 & 63.36 & 64.56 & 61.37 & 70.52 & 68.71 & 62.47 \\
\rowcolor{red!20}
MMP & 51.03 & 49.95 & 55.50 & 51.98 & 57.72 & 52.58 & 69.91 & 71.31 & 69.37 & 68.12 & 67.51 & 71.41 & 70.03 & 70.58 & 71.41 & 60.12 \\
\rowcolor{red!20}
PPAR & 53.74 & 48.42 & 57.76 & 49.45 & 61.78 & 63.22 & 68.37 & 69.88 & 67.75 & 65.29 & 66.43 & 68.88 & 69.43 & 68.83 & 68.21 & 66.31 \\
\midrule
\rowcolor{blue!20}
COLLAB & 49.72 & 51.38 & 54.62 & 51.41 & 36.47 & 38.18 & 44.91 & 45.44 & 60.58 & 51.85 & 48.13 & 72.45 & 54.32 & 71.01 & 69.34 & 46.77 \\
\rowcolor{blue!20}
IMDB-B & 51.75 & 52.83 & 52.98 & 51.79 & 40.89 & 45.64 & 68.00 & 63.88 & 61.47 & 53.31 & 65.27 & 70.12 & 65.94 & 69.82 & 66.68 & 59.25 \\
\rowcolor{blue!20}
REDDIT-B & 48.36 & 46.19 & 49.50 & 49.84 & 60.32 & 52.51 & 84.49 & 82.64 & 82.1 & 80.32 & 89.92 & 85.24 & 78.87 & 87.43 & 89.43 & 63.42 \\
\rowcolor{blue!20}
ENZYMES & 52.45 & 49.82 & 53.75 & 51.03 & 60.97 & 53.94 & 62.73 & 63.09 & 62.44 & 61.75 & 63.45 & 64.58 & 63.44 & 68.56 & 64.58 & 52.10 \\
\rowcolor{blue!20}
PROTEINS & 49.43 & 61.24 & 53.85 & 65.75 & 61.15 & 52.78 & 72.61 & 72.60 & 76.46 & 77.29 & 72.89 & 75.86 & 77.43 & 76.49 & 76.02 & 68.81 \\
\rowcolor{blue!20}
DD & 47.69 & 75.29 & 47.98 & 70.49 & 70.33 & 42.67 & 76.43 & 65.41 & 79.08 & 80.76 & 77.76 & 74.53 & 76.54 & 78.84 & 79.91 & 60.49 \\
\rowcolor{blue!20}
BZR & 46.67 & 59.08 & 51.16 & 51.71 & 41.50 & 45.42 & 68.93 & 67.81 & 69.13 & 68.55 & 51.89 & 80.79 & 68.23 & 77.69 & 73.28 & 65.94 \\
\rowcolor{blue!20}
AIDS & 50.93 & 52.01 & 52.56 & 61.42 & 87.2 & 97.96 & 95.44 & 98.8 & 96.89 & 96.93 & 99.36 & 97.6 & 98.02 & 99.21 & 97.1 & 70.82 \\
\rowcolor{blue!20}
COX2 & 52.15 & 52.48 & 53.34 & 49.56 & 49.11 & 48.61 & 59.68 & 59.38 & 57.81 & 58.93 & 59.81 & 72.35 & 64.13 & 64.36 & 63.19 & 54.73 \\
\rowcolor{blue!20}
NCI1 & 51.39 & 50.22 & 54.18 & 50.41 & 45.11 & 61.88 & 43.3 & 46.44 & 69.46 & 65.29 & 75.75 & 74.32 & 68.32 & 69.13 & 61.58 & 58.74 \\
\rowcolor{blue!20}
DHFR & 48.31 & 52.79 & 50.3 & 51.64 & 45.58 & 63.15 & 58.21 & 57.01 & 61.09 & 61.79 & 59.82 & 72.87 & 61.25 & 63.23 & 64.48 & 53.23 \\
\midrule
\rowcolor{green!20} 
IMDB-M & 49.8 & 51.23 & 53.45 & 53.03 & 56.26 & 51.32 & 74.45 & 78.62 & 80.98 & 81.25 & 66.73 & 71.1 & 78.28 & 80.23 & 80.94 & 52.67 \\
\rowcolor{green!20} 
ENZYMES & 52.53 & 53.36 & 53.92 & 51.9 & 46.01 & 33.52 & 59.76 & 63.23 & 61.77 & 59.36 & 67.18 & 62.42 & 56.95 & 64.31 & 63.84 & 54.48 \\
\rowcolor{green!20} 
AIDS & 51.18 & 51.69 & 52.28 & 50.95 & 44.33 & 63.27 & 97.11 & 98.48 & 95.68 & 94.33 & 98.95 & 96.82 & 95.42 & 99.1 & 99.27 & 94.58 \\
\rowcolor{green!20} 
BZR & 43.34 & 52.43 & 49.76 & 52.16 & 64.29 & 64.65 & 78.98 & 76.01 & 87.27 & 80.55 & 81.86 & 89.11 & 83.21 & 96.32 & 95.16 & 65.26 \\
\rowcolor{green!20} 
ESOL & 52.99 & 52.63 & 52.13 & 52.28 & 58.12 & 99.64 & 78.66 & 79.66 & 86.7 & 90.55 & 88.32 & 91.43 & 89.3 & 92.41 & 91.98 & 75.65 \\
\rowcolor{green!20} 
TOX21 & 53.73 & 51.87 & 53.5 & 52.25 & 97.04 & 66.53 & 66.85 & 64.85 & 67.29 & 69.8 & 68.91 & 66.72 & 72.51 & 68.24 & 66.7 & 72.34 \\
\rowcolor{green!20} 
BBBP & 54.15 & 53.11 & 54.62 & 53.48 & 63.27 & 32.37 & 69.18 & 67.33 & 78.83 & 77.69 & 78.93 & \textbf{89.88} & 79.07 & 80.17 & 81.44 & 55.69 \\
\rowcolor{green!20} 
PTC\_MR & 51.52 & 55.87 & 54.03 & 52.12 & 55.88 & 53.78 & 78.1 & 79.74 & 79.27 & 77.54 & 62.51 & \textbf{84.63} & 80.12 & 79.44 & 82.05 & 58.28 \\
\rowcolor{green!20} 
FREESOLV & 50.06 & 54.76 & 51.98 & 53.24 & 44.98 & 49.57 & 67.05 & 66.01 & 66.98 & 68.92 & 64.38 & \textbf{78.12} & 67.32 & 69.89 & 71.58 & 60.12 \\
\rowcolor{green!20} 
CLINTOX & 50.85 & 51.74 & 52.66 & 51.54 & 55.62 & 56.45 & 59.65 & 54.17 & 61.21 & 58.31 & 59.3 & \textbf{72.15} & 63.42 & 70.21 & 69.28 & 50.79 \\

\midrule
\rowcolor{yellow!20} 
HIV-Size       & 48.94 & 49.96 & 66.11 & 45.10 & 31.39 & 32.67 & 26.73 & 35.80 & 38.55 & 42.94 & \textbf{96.34} & 91.86 & 47.56 & 56.23 & 74.12 & 68.31 \\
\rowcolor{yellow!20} 
ZINC-Size      & 48.66 & 50.12 & 50.58 & 48.96 & 53.07 & 53.47 & 52.61 & 53.46 & 54.22 & 54.21 & 59.41 & 57.29 & 52.53 & 58.78 & 68.43 & 55.63 \\
\rowcolor{yellow!20} 
HIV-Scaffold   & 49.36 & 48.43 & 44.72 & 54.57 & 58.78 & 58.74 & 61.00 & 59.26 & 56.82 & 54.38 & 58.05 & 70.93 & 63.23 & 59.49 & 62.28 & 53.48 \\
\rowcolor{yellow!20} 
ZINC-Scaffold  & 51.12 & 46.66 & 51.17 & 53.28 & 54.77 & 55.17 & 54.04 & 55.80 & 51.87 & 50.12 & 56.79 & 59.24 & 55.79 & 55.73 & 56.39 & 55.62 \\
\rowcolor{yellow!20} 
IC50-Size      & 67.08 & 59.35 & 90.76 & 52.49 & 32.61 & 36.15 & 24.44 & 30.96 & 42.58 & 41.29 & 97.36 & 81.43 & 39.63 & 50.37 & 50.71 & 45.24 \\
\rowcolor{yellow!20} 
EC50-Size      & 70.50 & 59.33 & 92.29 & 49.36 & 29.71 & 32.60 & 22.83 & 27.68 & 41.37 & 39.42 & 97.74 & 77.12 & 39.23 & 55.84 & 56.58 & 59.49 \\
\rowcolor{yellow!20} 
IC50-Scaffold  & 66.33 & 60.95 & 88.49 & 58.56 & 36.96 & 38.67 & 34.60 & 38.82 & 44.56 & 42.97 & 96.00 & 77.58 & 38.43 & 57.96 & 56.62 & 59.68 \\
\rowcolor{yellow!20} 
EC50-Scaffold  & 64.95 & 62.78 & 86.03 & 55.27 & 27.88 & 30.36 & 31.28 & 32.35 & 51.92 & 48.43 & 94.18 & 74.65 & 40.98 & 66.52 & 58.29 & 54.24 \\
\rowcolor{yellow!20} 
IC50-Assay     & 54.47 & 53.13 & 59.18 & 52.11 & 51.23 & 51.42 & 51.15 & 51.93 & 52.61 & 49.87 & 68.78 & 65.99 & 52.12 & 54.25 & 53.74 & 57.11 \\
\rowcolor{yellow!20} 
EC50-Assay     & 49.08 & 46.66 & 48.43 & 45.32 & 47.80 & 47.81 & 47.80 & 46.02 & 56.11 & 52.44 & 69.31 & 82.97 & 54.34 & 66.71 & 65.57 & 58.96 \\
\midrule
\rowcolor{gray!20} 
Ave. & 12.09 & 11.94 & 10.46 & 11.77 & 11.84 & 11.51 & 8.20 & 8.34 & 6.74 & 8.29 & 4.97 & 3.40 & 7.20 & 4.57 & 4.60 & 10.20 \\
\rowcolor{gray!20} 
Rank. & 16 & 15 & 11 & 13 & 14 & 12 & 7 & 9 & 5 & 8 & 4 & 1 & 6 & 2 & 3 & 10 \\
% Imp.  & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 &0 \\


\bottomrule
\end{tabular}
}
\end{table}


\subsection{Specialized Experiments in Near OOD and Far OOD settings (RQ2)}
To rigorously evaluate the performance of GLOD and GLAD methods in distinguishing between near-OOD and far-OOD conditions, we implemented a distinct partitioning strategy as detailed in Table~\ref{tab:near_far} and Fig.~\ref{fig:near_far}. The following key findings emerge from our evaluations.

$\rhd$ \textbf{Larger Differences from ID Samples Facilitate Detection.}

From Fig.~\ref{fig:near_far}, it is evident that models generally perform better in detecting far-OOD samples compared to near-OOD samples. This trend is consistent across various datasets. For instance, in the AIDS dataset, models like GLocalKD, OCGTL, and SIGNET achieve higher AUROC values for far-OOD conditions than for near-OOD. Similar patterns are observed in the BZR and ENZYMES datasets, where most models display better performance in far-OOD scenarios. This consistent performance discrepancy underscores the challenge of detecting near-OOD samples that closely resemble the ID data, highlighting the need for enhanced model sensitivity to subtle deviations.

$\rhd$ \textbf{Limitations of GLAD and GLOD Methods in Specialized Scenarios.}
Despite the overall effectiveness of GLAD and GLOD methods, there are notable limitations in their performance, particularly in specialized scenarios. Preliminary findings from the Class-based Anomaly Scenario of GLAD reveal that GLOD methods like GOOD-D and GraphDE exhibit significant performance gaps between near-OOD and far-OOD conditions. This suggests that when OOD samples are similar to ID samples, the detection capability of GLOD methods is significantly compromised. This limitation is even more pronounced in the Size-based Scenario of GLOD tasks, where GLAD methods underperform significantly compared to simpler methods. In these scenarios, GLAD methods struggle with size-based deviations, resulting in substantial performance gaps. These findings highlight the need for more adaptable models that can effectively handle near-OOD samples and specialized scenarios to improve overall detection performance.

$\rhd$ \textbf{Varying Sensitivity Across Datasets.}
The AUROC comparison of models on different datasets, as shown in Fig.~\ref{fig:near_far}, indicates that different models exhibit varying sensitivity to anomalies across different datasets. For example, in the AIDS dataset, models like GLocalKD and OCGTL show high sensitivity to near and far-OOD samples, whereas in the BZR dataset, models such as GOOD-D and SIGNET perform relatively better. However, in the ENZYMES dataset, the performance of these models is more variable, with no single model consistently outperforming the others. This variability in performance suggests that the effectiveness of GLOD and GLAD methods is highly dependent on the specific characteristics of the dataset. It highlights the importance of evaluating models across diverse datasets to understand their strengths and limitations comprehensively.

The findings from RQ2 emphasize the importance of evaluating GLOD and GLAD methods under both near-OOD and far-OOD conditions. Performance discrepancies highlight the need for developing more adaptable and resilient models. Our evaluation framework provides a comprehensive understanding of model capabilities in handling varying degrees of OOD data. Additionally, the varying sensitivity across different datasets underscores the necessity for thorough testing in multiple contexts to ensure generalizability and robustness.

\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{Figs/near_far.pdf}
    \caption{Near and Far OOD performance comparison.}
    \label{fig:near_far}
\end{figure}

\subsection{Impact of OOD Contamination in ID Training on Model Performance (RQ3)}
To investigate the robustness of GLOD and GLAD methods against the contamination of the ID training set with OOD samples, we conducted a series of experiments where varying proportions of OOD samples were added to the ID training data. This setup allows us to systematically explore how the inclusion of OOD samples affects the models' ability to identify and differentiate true OOD instances during testing accurately.

$\rhd$ \textbf{Performance Degradation with Increasing OOD Contamination.}
From our experiments, it is clear that as the proportion of OOD samples in the ID training set increases, the performance of both GLOD and GLAD methods generally deteriorates. This trend is evident across multiple datasets and models, as shown in Fig.\ref{fig:perturbations}. For example, in the PROTEINS, BZR, and COX2 datasets, we observe that models such as GLocalKD, OCGTL, SIGNET, GOOD-D, and others show a consistent decrease in AUROC values as the proportion of OOD contamination increases from 0\% to 30\%. This decline in performance suggests that the presence of OOD samples in the training data introduces noise and confounds the models, making it increasingly difficult for them to distinguish between ID and OOD samples during testing.

$\rhd$ \textbf{Robustness and Sensitivity to Perturbations.}
Interestingly, some models exhibit notable robustness to OOD contamination. For instance, GLADC shows minimal performance degradation across all datasets even as OOD perturbation levels increase. This indicates a high degree of robustness, making GLADC particularly reliable in scenarios where OOD contamination is likely.
Similarly, CVTGOD demonstrates impressive stability in the BZR dataset. As shown in Fig.~\ref{fig:perturbations}, the performance of CVTGOD remains relatively constant from 10\% to 30\% OOD contamination, suggesting the presence of a perturbation threshold beyond which the model's performance does not significantly degrade. This characteristic makes CVTGOD a robust choice for datasets with varying levels of contamination.
Conversely, some models are highly sensitive to perturbations. For example, OCGTL's performance in the PROTEINS dataset declines sharply as the level of OOD contamination increases. This significant drop indicates a high sensitivity to noise, highlighting the need for improving the robustness of such models to ensure reliable performance in real-world scenarios where data contamination is common.

The inclusion of OOD samples in the ID training set significantly impacts the performance and robustness of GLOD and GLAD methods. This study underscores the importance of developing strategies to mitigate the effects of OOD contamination during training. By addressing these challenges, we can enhance the development of more resilient models capable of maintaining high performance across diverse and challenging scenarios. The variability in robustness across different models and datasets emphasizes the need for comprehensive testing to identify and address potential weaknesses in anomaly detection approaches.


\subsection{Computational Efficiency of GLOD and GLAD Methods (RQ4)}

$\rhd$ \textbf{Time Efficiency.}

$\rhd$ \textbf{Resource Usage.}



\begin{figure}[ht]
    \centering
    \includegraphics[width=\textwidth]{Figs/perturbations.pdf}
    \caption{Performance of models under different perturbation levels.}
    \label{fig:perturbations}
\end{figure}



\begin{figure}[ht]
    \centering
    \subfigure[Memory Usage]{\includegraphics[width=0.45\textwidth]{Figs/memory_usage.pdf}\label{fig:memory_usage}}
    \hspace{0.05\textwidth}
    \subfigure[Time Usage]{\includegraphics[width=0.45\textwidth]{Figs/time_usage.pdf}\label{fig:time_usage}}
    \caption{Comparison of Memory and Time Usage.}
    \label{fig:usage}
\end{figure}



==> Tables/datasets_v1.tex <==
\begin{table}[h!]
\centering
\caption{Dataset Details}
\resizebox{\textwidth}{!}{%
\begin{tabular}{lllcccccc}
\toprule
\textbf{Dataset Type} & \textbf{ID Dataset} & \textbf{OOD Dataset} & \textbf{Graph Type} & \textbf{OOD Type} & \textbf{\# ID Train} & \textbf{\# ID Test} & \textbf{\# OOD Test} \\
\midrule
\multirow{4}{*}{Real Anomaly} 
& p53 & - & Molecules &Inherent  &8088 &241 &28 \\
& HSE & - & Molecules &Inherent &423 &257 &10 \\
& Tox21\_MMP & - & Molecules &Inherent &6170 &200 &38   \\
& PPAR-gamma & - & Molecules &Inherent & 219 & 252  & 15\\
\midrule
\multirow{11}{*}{Class-based Anomaly} 
& COLLAB &- & Social Networks & Unseen Classes &1920 &480 &520 \\
& IMDB-BINARY &- & Social Networks &Unseen Classes &400 &100 &100 \\
& REDDIT-BINARY &- & Social Networks &Unseen Classes &800 &200 &200 \\
& ENZYMES &- & Proteins &Unseen Classes &400 &100 &20 \\
& PROTEINS & -& Proteins &Unseen Classes &360 &90 &133 \\
& DD &- & Proteins &Unseen Classes  &390 &97 &139 \\
& BZR & -& Molecules &Unseen Classes &69 &17 &64 \\
& AIDS &- & Molecules &Unseen Classes &1280 &320 &80  \\
& COX2 & -& Molecules &Unseen Classes &81 &21 &73 \\
& NCI1 & -& Molecules &Unseen Classes &1646 &411 &411 \\
& DHFR & -& Molecules &Unseen Classes &368 &93 &59  \\
\midrule
\multirow{10}{*}{Inter-Dataset Shift} 
& IMDB-MULTI & IMDB-BINARY & Social Networks &Unseen Datasets  &1350 &150 &150 \\
& ENZYMES & PROTEINS & Proteins &Unseen Datasets &540 &60 &60  \\
& AIDS & DHFR & Molecules &Unseen Datasets &1800 &200 &200 \\
& BZR & COX2 & Molecules &Unseen Datasets &364 &41 &41 \\
& ESOL & MUV & Molecules &Unseen Datasets &1015 &113 &113 \\
& TOX21 & SIDER & Molecules &Unseen Datasets &7047 &784 &784 \\
& BBBP & BACE & Molecules &Unseen Datasets &1835 &204 &204 \\
& PTC\_MR & MUTAG & Molecules &Unseen Datasets &309 &35 &35 \\
& FREESOLV & TOXCAST & Molecules &Unseen Datasets &577 &65 &65 \\
& CLINTOX & LIPO & Molecules &Unseen Datasets &1329 &148 &148 \\
\midrule
\multirow{10}{*}{Intra-Dataset Shift} 
& GOOD-HIV-Size & -& Molecules &Size &1000 &500 &500  \\
& GOOD-ZINC-Size & -& Molecules &Size &1000 &500 &500  \\
& GOOD-HIV-Scaffold & -& Molecules &Scaffold &1000 &500 &500  \\
& GOOD-ZINC-Scaffold & -& Molecules &Scaffold &1000 &500 &500  \\


& DrugOOD-IC50-Size	 & -& Molecules & Size &1000 &500 &500  \\
& DrugOOD-EC50-Size	 & -& Molecules & Size &1000 &500 &500  \\
& DrugOOD-IC50-Scaffold & -& Molecules & Scaffold &1000 &500 &500  \\
& DrugOOD-EC50-Scaffold & -& Molecules & Scaffold &1000 &500 &500  \\
& DrugOOD-IC50-Assay & -& Molecules & Protein Target &1000 &500 &500  \\
& DrugOOD-EC50-Assay & -& Molecules & Protein Target &1000 &500 &500  \\
\bottomrule
\end{tabular}
}
\label{tab:dataset}
\end{table}
